Leveraging Unpaired Data for Vision-Language Generative Models via Cycle Consistency

Current vision-language generative models rely on expansive corpora of paired image-text data to attain optimal performance and generalization capabilities. However, automatically collecting such data (e.g. via large-scale web scraping) leads to low quality and poor image-text correlation, while human annotation is more accurate but requires significant manual effort and expense. We introduce $\textbf{ITIT}$ ($\textbf{I}$n$\textbf{T}$egrating $\textbf{I}$mage $\textbf{T}$ext): an innovative training paradigm grounded in the concept of cycle consistency which allows vision-language training on unpaired image and text data. ITIT is comprised of a joint image-text encoder with disjoint image and text decoders that enable bidirectional image-to-text and text-to-image generation in a single framework. During training, ITIT leverages a small set of paired image-text data to ensure its output matches the input reasonably well in both directions. Simultaneously, the model is also trained on much larger datasets containing only images or texts. This is achieved by enforcing cycle consistency between the original unpaired samples and the cycle-generated counterparts. For instance, it generates a caption for a given input image and then uses the caption to create an output image, and enforces similarity between the input and output images. Our experiments show that ITIT with unpaired datasets exhibits similar scaling behavior as using high-quality paired data. We demonstrate image generation and captioning performance on par with state-of-the-art text-to-image and image-to-text models with orders of magnitude fewer (only 3M) paired image-text data.

==> intro.tex <==
\section{Introduction}
Image-text multimodal training has gained remarkable attention in recent years. Models for text-to-image generation show the impressive ability to synthesize realistic images from textual prompts \citep{rombach2022high, chang2023muse, saharia2022photorealistic, yu2022scaling, ramesh2021zero}. Similarly, image-to-text models have demonstrated advanced image comprehension capabilities by providing precise descriptions of input images \citep{chen2023pali, wang2022git, li2022blip, li2023blip, alayrac2022flamingo, wang2022simvlm}. 
Training these models to exceptional performance demands datasets comprising hundreds of millions to billions of \emph{paired} image-text samples  \citep{schuhmann2022laion}. 
The collection of very large paired datasets comes at a considerable cost as well as concerns of low quality \citep{jia2021scaling}. On the other hand, diverse and vast unimodal images or texts datasets remain unused in current generative vision-language training \citep{raffel2020exploring,sun2017revisiting,zhai2022scaling}. This raises a natural question: can we leverage \textit{unpaired} image and text data to facilitate generative vision-language training?
% \han{Since it might have many meanings for vision-language training, Should we define this or make it more specific, like generative vision-language training?}

\begin{figure}[t]
\begin{center}
\vspace{-10pt}
\includegraphics[width=1.0\linewidth]{teaser}

\vspace{-10pt}
\end{center}
\caption{Overview of \name. For unpaired data, \name~first generates the image/text counterpart, and then uses these generated counterparts to reconstruct the original text or image.}\label{fig:teaser}
\vspace{-10pt}
\end{figure}

The major problem with using unpaired data during vision-language training is the lack of supervision. Generative vision-language training needs paired text to supervise image-to-text captioning, and paired images to supervise text-to-image generation. To solve this problem, we introduce \name, a novel training paradigm that significantly reduces the reliance on paired image-text data, favoring instead the utilization of unpaired image-only and text-only data. As shown in \Cref{fig:teaser}, the core principle underlying \name~is the use of \emph{cycle consistency} losses between cycle-generated images/texts and their corresponding original inputs to provide supervision for image-only and text-only data during training.

% Our model unifies image-to-text (I2T) and text-to-image (T2I) generation, 
To enable cycle training, we first unify image-to-text (I2T) and text-to-image (T2I) generation in the same framework, with a bi-directional image-text encoder and disjoint image and text decoders. We tokenize images into discrete visual tokens \citep{van2017neural} and combine them with text embeddings from a pre-trained T5 model \citep{raffel2020exploring} as input to the joint image-text encoder. For I2T generation, we employ an autoregressive text decoder \citep{wang2022git}, while for T2I generation we use a non-autoregressive parallel image decoder \citep{chang2023muse}, which is an order of magnitude faster than autoregressive image decoders such as \cite{yu2022scaling}. 

During training, \name~utilizes a small set of paired image-text data to achieve reasonable text-to-image and image-to-text generation performance, and align concepts in the image and text spaces. Simultaneously, for unpaired image (text) data, \name~generates corresponding text (image) counterparts and employs them as inputs to reconstruct the input image (text): this corresponds to a full cycle loss. We consider two kinds of full cycles: T2I2T (starting with an unpaired text sample); and I2T2I (starting with an unpaired image sample). For both modalities, we employ 
% \sangnie{is autoregressive loss a 'masking loss' for text:?} 
cross-entropy loss for the reconstruction, which enable a simple, unified approach for cycle consistency.
% The intermediate image or text sample is generated and used as part of the full cycle. 
ITIT enables us to leverage unpaired image and text data to provide informative supervision signals for training.

We evaluate the performance of \name~on standard image-to-text and text-to-image generation benchmarks and demonstrate that, by leveraging unpaired data and cycle consistency, \name~attains performance levels similar to a non-cycle baseline. However, \name~uses significantly up to 2 orders of magnitude lower paired data. Furthermore, \name~scales similarly with unpaired data as the baseline does with equivalent amounts of paired data, while being much more robust to low data quality. We also compare \name~with state-of-the-art methods and show that we can achieve comparable performance on common text-to-image and image-to-text benchmarks with substantially lesser paired data. Our contributions are summarized as follows:

% With only 3 million paired data from CC3M and 111 million unpaired data from WebLI, \name~ trained on a ViT-H model \citep{vit} achieves 10.4 zero-shot FID on MS-COCO and 38.2 zero-shot CIDEr on COCO Captions. This compares very favorably to, for example, the COBIT-Large model \citep{you2023cobit} which has a similar number of parameters, but uses 3 \emph{orders of magnitude} more paired data (see Table \ref{tab:sota}).

% \yonglong{Overall, I think we can largely abbreviate the above paragraph, and absorb the key things into the following bullets}

\begin{itemize}
    % \item  \han{I think this can be merged with the second one. After all, many previous work unifies t2i and i2t. Also we might add another contribution saying, we conduct detailed analysis on our model with cycle consistency and find.... (the interesting observation that the samples are more consistent after many cycles),  not just about improvement on FID or CIDEr.}
    \item We introduce a framework that unifies text-to-image and image-to-text generation, and propose \name, a novel technique that enforces consistency between cycle-generated images/text and their corresponding originals. This approach allows the training of image-to-text and text-to-image models using unpaired image and text data.
    \item We comprehensively evaluate the proposed \name~framework and the image-text cycle consistency method, and demonstrate that they significantly enhance model performance.
    \item We show that \name~can achieve performance on par with state-of-the-art methods on common text-to-image and image-to-text benchmarks with much lesser ($\sim$100x) paired data. When scaling up training data to improve model efficacy, we show that we can add only unpaired examples using our framework and achieve similar performance as scaled-up paired data, without the downsides of significant manual effort and poor pairing quality.
\end{itemize}

==> method.tex <==
\section{Method}
\name~is the first framework that enables vision-language training on unpaired image-only and text-only data. It uses a simple yet effective architecture: a unified image-text encoder and two separate image and text decoders. This design seamlessly enables text-to-image and image-to-text generation in the same framework, which paves the way for text-image-text (T2I2T) and image-text-image (I2T2I) training. 
% During such training, \name~first uses text-only and image-only data to synthesize its image/text counterparts. It then uses the synthesized image/text as input and forces them to generate the original text/image. 
\sangnie{should add somewhere that we use masked image modeling for image generation, and autoregressive for text}
Below, we describe each component of our ITIT framework and the cycle-consistency training paradigm in detail. 
\subsection{Unified Image-Text Generation Framework}
\noindent\textbf{Architecture.} 
% To seamlessly enable text-to-image and image-to-text generation in the same framework, we design a simple yet effective network architecture named ITIT (InTerleaving Image Text). 
% As shown in \Cref{fig:model}, ITIT is composed of a unified image-text encoder, and two separate image and text decoders. Raw text and images are first encoded with a pre-trained T5 encoder and a pre-trained VQ-tokenizer respectively. 
We first obtain text tokens $T=[t_l]_{l=1}^L$ using a pre-trained T5 encoder \sangnie{cite} on the raw text. Similarly, raw images are passed through a pre-trained VQ-tokenizer (\sangnie{cite}) to output image tokens $I=[i_k]_{k=1}^K$. $L$ and $K$ are the respective token sequence lengths.
The image tokens $I$ are then embedded (\sangnie{how}) and concatenated with the T5 text features $T$ as the input to the image-text encoder. Modality-specific decoders then operate on the encoded image-text features to generate either text or image tokens.

\noindent\textbf{T2I Training.} 
% Let $Y=[y_i]_{i=1}^N$ denote the latent image tokens obtained from the tokenizer, where $N$ is the token sequence length, and $M=[m_i]_{i=1}^N$ denotes a corresponding binary mask determining which tokens are to be masked. Let $T=[t_i]_{i=1}^K$ denotes the text paired with the image. 
We use masked image modeling for image generation, where the training objective is to reconstruct masked image tokens using the unmasked tokens and the paired text features. We denote the binary mask determining which image tokens are masked by $M=[m_k]_{k=1}^N$. We add a cross-entropy loss between the ground-truth one-hot image tokens and the output of the image decoder. Specifically,
\begin{equation}
    \mathcal{L}_{T2I} = -\mathbb{E}_{(I, T)\in \mathcal{D}} \big(\sum_{\forall k, m_k=1} \log p(i_k|I_{M}, T)\big),
\end{equation}
where $I_M$ are the (subset of) \emph{unmasked} tokens in $I$ and $p(i_k|I_{M}, T)$ is the probability predicted by the encoder-decoder network (the `logits' layer).
Further, to enable classifier-free guidance for generation, we set the text to be empty with 50\% probability.

\noindent\textbf{I2T Training.} When using empty text features for classifier-free guidance, we use the features generated by the image-text encoder to train our text decoder. We use a language modeling (LM) loss to train our text decoder. Setting $t_0$ to be the [BOS] token,
\begin{equation}
    \mathcal{L}_{I2T} = -\mathbb{E}_{(I, T)\in \mathcal{D}} \big( \sum_{l=1}^{L} \log p(t_l|I_{M}, t_0, \cdots, t_{l-1} )\big),
\end{equation}

which is a CE loss with label smoothing 0.1 \tianhong{what is label smoothing here?}. Similar to GIT (\cite{wang2022git}), we found that the image-text encoder should receive smaller gradient than the text decoder \tianhong{why? details? ablations?}. Therefore, we scale down the gradient backpropagated from the text decoder to the image-text encoder by 0.1. In practice, this is simply implemented by $z = 0.1z + \text{stopgrad}(0.9z)$ where $z$ denotes the output of the image-text encoder.

\noindent\textbf{T2I Inference.} Similar to Muse (\cite{chang2023muse}), we use parallel decoding with classifier-free guidance to generate an image from a text prompt. We start with a blank image, with all the tokens masked out, and pass these concatenated with the text prompt tokens. At each iteration, the decoder predicts a conditional logit $l_c$ and an unconditional logit $l_u$ for each masked token. The final logits $l_g$ are formed by moving away from $l_u$ by the guidance scale $t_g$ \sangnie{use another variable for this unless it is standard (t is already text)}: $l_g = (1+t)l_c - t_gl_u$. We then sample the top-k tokens with the highest predicted probability, and replace the corresponding masked tokens with these sampled predicted tokens. The number of masked tokens to be replaced in each iteration follows a cosine function
% , i.e., we replace fewer masked tokens in the early iterations and more masked tokens at later iterations
. We use a total of 24 steps to generate an image. \sangnie{do we need all details of image generation here or can we just refer to Muse? }

\noindent\textbf{I2T Inference.} To generate captions for an image, we first extract visual features from the image (and empty text) using the image-text encoder. Then we auto-regressively generate the tokens conditioning on the visual features and previous generated tokens. Following GIT (\cite{wang2022git}), we use beam search to pick the tokens with a beam size of 4.

\subsection{Cycle Consistency Training}
Our cycle consistency training paradigm allows training with image-only and text-only data. The key idea is to first synthesize the corresponding text/image from the image-only or text-only data, and then use the synthesized data as input to reconstruct the original image/text. This allows us to apply cycle consistency supervision on image-only and text-only data.

\noindent\textbf{Image-Text-Image (I2T2I) Consistency.}
Our I2T2I training pipeline is shown in \Cref{fig:i2t2i}. At each training iteration, we first synthesize text $T$ using our I2T inference pipeline from the input image $I$. Then we use the I2T training pipeline to autoregressively predict $\Tilde{t_i}$ from $t_0, \cdots, t_{i-1}$ and $I$. We then mask $I$, take the predicted $\Tilde{T}$ and go through the T2I pipeline to predict the masked image tokens. Therefore, the I2T2I cycle-consistency loss can be formulated as follows:

\begin{equation}
    \mathcal{L}_{I2T2I} = -\mathbb{E}_{Y\in \mathcal{D}_{image}} \big(\sum_{\forall i, m_i=1} \log p(y_i|Y_{M}, \Tilde{T})\big),
\end{equation}
Such loss is very similar to the above T2I loss, except for $\Tilde{T}$ is not drawn from the image-text joint distribution, but is synthesized from $Y$.

\noindent\textbf{Text-Image-Text (T2I2T) Consistency.}
Our T2I2T training pipeline is shown in \Cref{fig:t2i2t}. At each training iteration, we first synthesize image $Y$ using our T2I inference pipeline from the input text $T=[t_l]_{l=1}^L$. Then we randomly masked out $Y$, and use the T2I training pipeline to reconstruct it. We denote the reconstructed synthesized image as $\Tilde{Y}$. Then $\Tilde{Y}$ goes through the I2T pipeline to predict the text. Therefore, the T2I2T cycle-consistency loss can be formulated as follows:

\begin{equation}
    \mathcal{L}_{T2I2T} = -\mathbb{E}_{T\in \mathcal{D}_{text}} \big( \sum_{l=1}^{L} \log p(t_l|\Tilde{I}_{M}, t_0, \cdots, t_{l-1} )\big),
\end{equation}

Such loss is very similar to the above I2T loss, except for $\Tilde{Y}$ is not drawn from the image-text joint distribution, but is synthesized from $T$.

\noindent\textbf{Gradient Estimation.}
One challenge in our cycle training is that, $\Tilde{y_i}=\arg\max p(y_i|Y_M, T)$ and $\Tilde{t_i}=\arg\max p(t_i|Y_M, t_0, \cdots, t_{i-1})$, which is not derivable. To solve this, we use a straight-through estimation on the predicted logits to approximate the gradient. Specifically, we directly copy the gradient on the one-hot prediction to the predicted logits after softmax:  

\begin{equation}
\begin{split}
    \text{onehot}(\Tilde{y_i}) & = p(y_i | Y_M, T) + \text{stopgrad}(\text{onehot}(\Tilde{y_i}) - p(y_i | Y_M, T)) \\
     \text{onehot}(\Tilde{t_i}) & = p(t_i | Y_M, \Tilde{t_0}, \cdots, \Tilde{t_{i-1}}) + \text{stopgrad}(\text{onehot}(\Tilde{t_i}) - p(t_i | Y_M, \Tilde{t_0}, \cdots, \Tilde{t_{i-1}}))
\end{split}
\end{equation}

We show in \autoref{tab:ablation} that such gradient estimation helps improve both text-to-image and image-to-text performance.


